Finite Blocklength Regime Performance of Downlink Large Scale Networks

Some emerging 5G and beyond use-cases impose stringent latency constraints, which necessitates a paradigm shift towards finite blocklength performance analysis. In contrast to Shannon capacity-achieving codes, the codeword length in the finite blocklength regime (FBR) is a critical design parameter that imposes an intricate tradeoff between delay, reliability, and information coding rate. In this context, this paper presents a novel mathematical analysis to characterize the performance of large-scale downlink networks using short codewords. Theoretical achievable rates, outage probability, and reliability expressions are derived using the finite blocklength coding theory in conjunction with stochastic geometry, and compared to the performance in the asymptotic regime (AR). Achievable rates under practical modulation schemes as well as multilevel polar coded modulation (MLPCM) are investigated. Numerical results provide theoretical performance benchmarks, highlight the potential of MLPCM in achieving close to optimal performance with short codewords, and confirm the discrepancy between the performance in the FBR and that predicted by analysis in the AR. Finally, the meta distribution of the coding rate is derived, providing the percentiles of users that achieve a predefined target rate in a network.

==> Rate_Numerical_Results.tex <==

\subsection{Average Rate Numerical Results}\label{sec:rate_results}

{This subsection presents illustrative numerical results for the theoretical rate analysis provided in Sec.~\ref{sec:outage_capacity} and~\ref{sec:Constellation}, which are also validated via Monte Carlo simulation. The results presented investigate the effect of the blocklength $n$ and the FER $\epsilon$, the tightness of the proposed theoretical approximations, and the performance comparison between the FBR and the AR. Then, the performance of the MLPCM is investigated in comparison with the theoretical average coding rate.} 

%Simulations are carried out {first} for a {given distance between the UE and BS} (Theorem~\ref{Theorem:Avg_coding_Network}), then for a random {distance} (Corollary~\ref{Collary:Avg_Coding_Rate}). 


{Fig.~\ref{fig:n} plots the maximum average coding rate versus the average SNR {$\alpha_0$} for $n\hspace{-0.1cm}\in\{128,2048\}$, FER $\epsilon\in\{10^{-2},\ 10^{-5},\ 10^{-6}\}$, and $r_0=250$ m. Given a FER $\epsilon$, a gap exists between the average coding rate in the FBR and the AR. {The gap is around $1$ dB for $n=2048$ and is between $3$ and $5$ dB for $n=128$ at $\epsilon=10^{-5}$ and $10^{-6}$, respectively, which shows the severity of the SNR penalty in the FBR compared to the AR.} The figure shows the trade-off between reliability (represented by FER) and maximum average coding rate at a given $n$, {where} the maximum average coding rate decreases/increases as the FER decreases/increases. {For instance, to achieve a given maximum average coding rate at $n=128$ and FER $\epsilon=10^{-5}$, we need around $2$ dB more power compared with the same blocklength $n$ under the FER $\epsilon=10^{-2}$.} Furthermore, the impact of {small} $n$ becomes more {severe when the} FER $\epsilon$ is smaller, {resulting in rate degradation. Overall, this shows that} it is impractical to use results from the AR in the FBR.}

%{For instance, 5G is required to support packets of $512$ to $4096$ bits at an FER of $10^{-5}$~\cite{IoT,5G_1}, and this is expected to be as stringent as $10^{-9}$ in 6G}~\cite{5G_1}. This fact combined with the observations from the figure show that it is impractical to use {results from the AR in the FBR}.


The spatially averaged coding rate is depicted in Fig~\ref{fig:Capacity_r0} versus the transmit signal to noise power ratio $\frac{\mathcal{P}}{\sigma_w^2}$.\footnote{{The figure is plotted for a wide range of $\frac{\mathcal{P}}{\sigma_w^2}$ for illustrative purposes, bearing in mind that some values of $\frac{\mathcal{P}}{\sigma_w^2}$ in the plot may be impractical.}} The spatial randomness of the user location $r_0$ degrades the average coding rate compared to Fig.~\ref{fig:n}. The figure also shows that for high SNR (above $0$ dB), one cannot achieve the same rate and FER achieved at a given $n$ by decreasing $n$ and paying an SNR penalty. For instance, the rate achieved at $n=2048$, $\epsilon=10^{-5}$, $\text{SNR} = 10$ dB cannot be achieved at $n=128$ and $\epsilon=10^{-5}$. The only way to achieve such a rate at $n=128$ is by paying a FER penalty, which is impractical for applications that need high reliability. {Hence, it is important to select $n$} that balances the trade-off between reliability and coding rate. Similar to Fig.~\ref{fig:n}, Fig. \ref{fig:Capacity_r0} shows the importance of the results in this paper for characterizing {and optimizing} the performance of large-scale networks with latency-sensitive applications. 
 
  \begin{figure}[t]
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[height=0.8\linewidth,width=1\linewidth]{New_Figures/Modulation_fixed_r0.eps}
         \caption{$r_0=150\ m$, $n=128$, and $\epsilon=10^{-2}$.}
         \label{fig:Capacity_QAM}
     \end{subfigure}
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[height=0.8\linewidth,width=1\linewidth]{Figures2/Capacity_Random_r0.eps}
         \caption{Random $r_0$, $n=512$, and $\epsilon=10^{-2}$.}
         \label{fig:Modulation_r0}
     \end{subfigure}
     \caption{Average coding rate for M-QAM defined in~\eqref{eq:modulation} and~\eqref{eq:modulation_r0} at $\lambda=1\ \mathrm{BS/km^2}$ {and different values of $n$ and $\epsilon$}.}
     \label{fig:Modulation}
\end{figure}
Second, the maximum achievable coding rate for different modulation schemes, presented in Sec.~\ref{sec:Constellation}, is simulated for $r_0=150\ m$, $\lambda=1\ \text{BS}/ {\text{km}}^2$, blocklength $n=128$, and FER $\epsilon=10^{-2}$ {in Fig. \ref{fig:Modulation}}. Fig.~\ref{fig:Capacity_QAM} demonstrates the Monte Carlo simulated maximum achievable coding rate for QAM and the approximated maximum achievable coding rate using the Gamma approximation for various modulation orders, ${M}=\{2,4,8,16\}$,  {(Theorem~\ref{Theorem:ModulationCapacity}), along with the maximum achievable rate under Gaussian codebooks (Theorem \ref{Theorem:Avg_coding_Network})} versus $\alpha_0$. The approximated maximum achievable rate is very close to the simulated maximum achievable rate. Thus, the Gamma approximation in \eqref{eq:Gamma_app} {leads to a fairly tight approximation}. It is also observed that as the QAM modulation order increases, the performance improves towards the maximum average coding rate {(without Gaussian codebooks)} in a large-scale network {in the FBR (Theorem \ref{Theorem:Avg_coding_Network}).} Fig.~\ref{fig:Modulation_r0} plots, the average achievable rate versus a wide range of $\frac{\mathcal{P}}{\sigma_w^2}$ for illustrative purposes under a {Rayleigh distributed $r_0$}, { {QAM constellation with} $M=2,4,8,$ and $16$}, blocklenth $n=512$, and FER $\epsilon=10^{-2}${, showing a similar trend as} {for fixed $r_0$}. It is observed that the average achievable rate saturates at a rate of $\approx 2\ \text{bits/transmission}$ {for this choice of $\lambda$, $n$, and $\epsilon$, which is low compared to the case $r_0=150\ m$}. This performance is a consequence of averaging the performance of {nearby} UEs which have relatively strong received {desired signals} (high SINR) {and far away} UEs which suffer from more interference (low SINR).



{Finally,} considering the same setting in Fig.~\ref{fig:Capacity_QAM}, we simulate MLPCM with a QAM constellation for modulation orders $M=2,4,8,$ and $16$ in Fig.~\ref{fig:BPSK_QPSK_8QAM_16QAM}. {The simulations are performed by fixing the SNR and {increasing the coding rate until reaching} the FER $\epsilon$.} The achievable rates are plotted along with the theoretical expressions proposed in \eqref{eq:Capacity_FB_r_0}~and~\eqref{eq:modulation}. The figure shows that the achievable rates of the MLPCM scheme {with 2-QAM or 4-QAM approaches the theoretical rate of the corresponding QAM constellation.} However, for 8-QAM and 16-QAM, a gap of $\approx 2.5$ dB exists between the theoretical results and the simulation results{. Nonetheless, this SNR gap translates to a small rate gap of fractions of bits/transmission due to the slow increase of the rate versus SNR in the large-scale network which is caused by interference.} Fig.~\ref{fig:BPSK_QPSK_8QAM_16QAM} {thus validates that the theoretical performance under finite constellations can be approached using MLPCM, which validates the potential of MLPCM} for future technologies.
% Polar Codes
\begin{figure}[t]
    \centering
    \includegraphics[height=0.41\linewidth,width=0.55\linewidth]{Figures2/gamma_MLPCM.eps}
    \caption{The average coding rate versus $r_0^{-\eta}\alpha$ at $\lambda=1\ \mathrm{BS/km^2}$, $r_0=150\ m$, and $n=128$.}
    \label{fig:BPSK_QPSK_8QAM_16QAM}
\end{figure}

Next, rate outage probability, reliability, and meta-distribution analysis are provided.


==> Results.tex <==
\section{Simulation \& Results}\label{sec:Results}
In this section, the results of Sec.~\ref{sec:outage_capacity}~,~\ref{sec:Constellation}~and~\ref{sec:PolarCodes} are presented and discussed for the system model presented in Sec.~\ref{sec:system_model}. The average coding rate and outage probability for random exclusion region with radius $r_0$ is first presented for large-scale networks in a finite blocklength regime then the average coding rate of different modulation schemes for the large-scale networks is displayed for the same system model. finally, the average coding rate of polar codes for blocklength of $n$ and frame error probability $\epsilon$ is presented and compared to the average coding rate derived in Eq.~\ref{eq:Capacity_FB} and~\eqref{eq:modulation}. 

The approximation of the outage probability for the large-scale networks for mobile users provided in~\eqref{eq:outage_without_r_0} is plotted in Fig.~\ref{fig:Outage_App} and compared to the simulated outage probability for different blocklengths and frame error probabilities. As shown, the blocklength increases the approximation becomes more accurate, and the difference between the simulated curve and the theoretical curve. Moreover, as the frame error probability increases the outage probability decreases, allowing more errors to take place makes the system less in outage. 

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=1.2\linewidth]{Figures/Outage_with_variable_r_o_1e2.eps}
         \caption{$\epsilon=10^{-2}$}
         \label{fig:Outage_App_1e2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=1.2\linewidth]{Figures/Outage_with_variable_r_o_1e5.eps}
         \caption{$\epsilon=10^{-5}$}
         \label{fig:Outage_App_1e5}
     \end{subfigure}
     \caption{The outage probability of the large-scale network vs. \text{SINR} threshold $T$ at $\lambda=1\ \mathrm{BS/km^2}$, $n=128,\ 2048$, and (a) $\epsilon=10^{-2}$ (b) $\epsilon=10^{-5}$ }
     \label{fig:Outage_App}
\end{figure}
The average coding rate for large-scale networks in a finite blocklength regime for a mobile user presented in~\eqref{eq:Capacity_FB_r_0} is depicted in Fig~\ref{fig:Capacity_r0}. The mobility of the user degraded the average coding rate if compared to the results provided in~\cite{mypaper}. Moreover, the figure shows the average capacity and the average coding rate for different blocklengths. As shown in the figure, large blocklengths provide average rates close to average capacity. As the blocklengths get shorter, a gap occurs between the average capacity and the average coding rate. 


\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/Capacity_with_variable_r_o.eps}
    \caption{Average Coding Rate vs. \text{SNR} at $\lambda=1\ \mathrm{BS/km^2}$, $n=128,\ 512,\ 2048$, and $\epsilon=10^{-3}$}
    \label{fig:Capacity_r0}
\end{figure}


Next, the average coding rate for different modulation schemes. The Fig.~\ref{fig:Capacity_QAM},~\ref{fig:Capacity_PSK},~\ref{fig:Capacity_ASK} demonstrated the average coding rate for the QAM, PSK modulation, and the ASK modulation schemes respectively. Each figure presented various modulation orders for a modulation scheme. In Fig.~\ref{fig:Capacity_QAM}, The average capacity, i.e. infinite blocklength and vanishing frame error probability, and the average coding rate at a blocklength of $128$ and a frame error probability of $10^{-2}$ is plotted for modulation order of $2,\ 4,\ 8,\ 16$. As shown in the figure that there is a gap between the average capacity and the average coding rate using short codes, which makes the expressions more accurate to represent the finite blocklength regimes. In Fig.~\ref{fig:Capacity_PSK}, the average coding rate for the PSK modulation is plotted for different modulation orders $2,\ 4,\ 8,\ 16$. As depicted in the figure, as the modulation order increases, no significant increase in the average coding rate is observed. In other words, the rate of increase of the average rate with respect to the modulation order is not significant. In Fig.~\ref{fig:Capacity_ASK}, the average coding rate  for the ASK modulation is plotted for different modulation orders $2,\ 4,\ 8,\ 16$. As depicted in the figure, as the modulation order increases, the rate of increase of the average coding rate is not significant which makes the gap between the 16-QAM scheme and the average capacity is small ($~1dB$ at $15dB$). Hence, for systems with complexity constraints, the 16-QAM scheme would give a good performance without the need to move to higher-order modulation.


%% QAM Modulation


\begin{figure}[!htb]
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[height=0.85\linewidth,width=1\linewidth]{Figures/Capacity_QAM_128.eps}
         \caption{QAM}
         \label{fig:Capacity_QAM}
     \end{subfigure}
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[height=0.89\linewidth,width=1.1\linewidth]{Figures/Capacity_PSK_128.eps}
         \caption{PSK}
         \label{fig:Capacity_PSK}
     \end{subfigure}\\
     \begin{minipage}[b]{1\textwidth}
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[height=0.89\linewidth,width=1.1\linewidth]{Figures/Capacity_ASK_128.eps}
         \caption{ASK}
         \label{fig:Capacity_ASK}
     \end{subfigure}
     \end{minipage}
     \caption{The average coding rate for various modulation schemes of a large-scale network vs. \text{SNR} at $r_0=\ 150\ m$, $\lambda=1\ \mathrm{BS/km^2}$, $n=128$, and $\epsilon=10^{-2}$. (a) QAM (b) PSK (c) ASK }
     \label{fig:Modulation}
\end{figure}


The average coding rate for different modulation schemes is evaluated at specific $r_0$ in Fig.~\ref{fig:Modulation}. These expressions are evaluated at random $r_0$. As discussed in Sec.~\ref{sec:system_model}, the distance between the user and the serving BS follows a Rayleigh distribution. Hence, by averaging the coding rate with respect to the $r_0$, the average coding rate is provided for a mobile user. So, in Fig.~\ref{fig:Capacity_QAM_r_o}, the average coding rate for a mobile user using the QAM scheme is provided for modulation order of $2,\ 4,\ 8,\ 16$ for a blocklenth of $n=512$ and frame error probability $\epsilon=10^{-2}$. The trend found for the stationary user is the same for the mobile where the average coding rate increases as the modulation order increase but not as the rate of increase decreases as the modulation order increases. Moreover, in Fig.~\ref{fig:Capacity_PSK_r0},  for the PSK modulation is plotted for a mobile user for different modulation orders $2,\ 4,\ 8,\ 16$ for a blocklenth of $n=512$ and frame error probability $\epsilon=10^{-2}$. Also, the average coding rate for ASK modulation scheme is plotted for a mobile user in Fig.~\ref{fig:Capacity_ASK_r0} for a blocklenth of $n=512$ and frame error probability $\epsilon=10^{-2}$. 
%% QAM_ro

\begin{figure}[!htb]
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[height=0.9\linewidth,width=1\linewidth]{Figures/Capacity_QAM_ro_new.eps}
         \caption{QAM}
         \label{fig:Capacity_QAM_r_o}
     \end{subfigure}
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[height=0.89\linewidth,width=1.1\linewidth]{Figures/Capacity_PSK_r_0_new.eps}
         \caption{PSK}
         \label{fig:Capacity_PSK_r0}
     \end{subfigure}\\
     \begin{minipage}[b]{1\textwidth}
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[height=0.89\linewidth,width=1.1\linewidth]{Figures/Capacity_ASK_ro_new.eps}
         \caption{ASK}
         \label{fig:Capacity_ASK_r0}
     \end{subfigure}
     \end{minipage}
     \caption{The average coding rate of various modulation schemes for a large-scale network vs. \text{SNR} $\lambda=1\ \mathrm{BS/km^2}$, $n=512$, and $\epsilon=10^{-2}$. (a) QAM (b) PSK (c) ASK }
     \label{fig:Modulation_r0}
\end{figure}


The MLPCM for QAM is simulated for various modulation order. The average coding rate for MLPCM scheme is plotted with the theoretical curves in Fig.~\ref{fig:BPSK_QPSK_8QAM_16QAM}
The figures shows that that the MLPCM schemes gives a performance near the average coding rate for the BPSK and the 4-QAM. For higher order modulation as 8-QAM and 16-QAM, a gap of (~2.5 dB) occurs between the theoretical results and the simulation results of the MLPCM scheme but still can be considered close to the theoretical curves.
% Polar Codes
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/All.eps}
    \caption{The average coding rate of the large-scale network vs. \text{SNR} at $\lambda=1\ \mathrm{BS/km^2}$, $n=128$, and (a) BPSK \& QPSK (b) 8-QAM \& 16-QAM }
    \label{fig:BPSK_QPSK_8QAM_16QAM}
\end{figure}


==> draft_file.tex <==
After analyzing \eqref{LapTrans}, it was found that the coefficients $a_k$ rapidly decay, and the first few coefficients are dominant. Hence, the Gamma approximation could be used to approximate the PDF of the interference power $\mathcal{B}$ using moment matching as proposed in the following proposition.

\begin{Proposition}\label{Proposition:1} 
The interference power $\mathcal{B}$ can be approximated by a Gamma distribution $f_{\hat{\mathcal{B}}}(B;q,\theta)=\frac{B^{q-1} e^{\frac{-B}{\theta}}}{\Gamma(q) \theta^q}$ using moment matching where \textcolor{red}{$q=\frac{\mathbb{E}\{\mathcal{B}\}^2}{\mathbb{V}ar\{\mathcal{B}\}}=\frac{4 \pi \lambda r_0^2 (\eta-1)}{(\eta-2)^2}$}, \textcolor{red}{$\theta=\frac{\mathbb{V}ar\{\mathcal{B}\}}{\mathbb{E}\{\mathcal{B}\}}=\frac{(\eta-2)\mathcal{P}}{2(\eta-1)r_0^2}$} and the mean and variance of $\mathcal{B}$ are given by $\mathbb{E}\{\mathcal{B}\}=\frac{2 \pi\lambda r_0^2 \mathcal{P}}{r_0^{\eta} (\eta-2)}$ and $\mathbb{V}ar\{\mathcal{B}\}=\frac{4 \pi \lambda r_0^2 \mathcal{P}^2}{r_0^{2\eta} (2\eta-2)\Gamma(3)}$.
\end{Proposition}

To verify this proposition, the exact PDF of the interference power $\mathcal{B}$ is plotted using numerical inversion of \eqref{LapTrans} and its Gamma approximation in Fig.~\ref{fig:gamma_vs_exact}. The figure shows that the Gamma approximation provides a tight and valid approximation.
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Figures/gamma_vs_exact2.eps}
    \caption{PDF of the Interference Power at $\mathcal{P}=10\ W$ $\lambda=10\ \text{BS}/\text{k}m^2$ and $r_0=250\ m$}
    \label{fig:gamma_vs_exact}
\end{figure}

